Co-Optimization of Design and Fabrication Plans for Carpentry

Past work on optimizing fabrication plans given a carpentry design can provide Pareto-optimal plans trading off between material waste, fabrication time, precision, and other considerations. However, when developing fabrication plans, experts rarely restrict to a single design, instead considering families of design variations, sometimes adjusting designs to simplify fabrication. Jointly exploring the design and fabrication plan spaces for each design is intractable using current techniques. We present a new approach to jointly optimize design and fabrication plans for carpentered objects. To make this bi-level optimization tractable, we adapt recent work from program synthesis based on equality graphs (e-graphs), which encode sets of equivalent programs. Our insight is that subproblems within our bi-level problem share significant substructures. By representing both designs and fabrication plans in a new bag of parts(BOP) e-graph, we amortize the cost of optimizing design components shared among multiple candidates. Even using BOP e-graphs, the optimization space grows quickly in practice. Hence, we also show how a feedback-guided search strategy dubbed Iterative Contraction and Expansion on E-graphs(ICEE) can keep the size of the e-graph manage-able and direct the search toward promising candidates. We illustrate the advantages of our pipeline through examples from the carpentry domain.

==> algo1.tex <==
% \begin{lstlisting}
% def ICEE (d, e):
%     # extract Pareto Front (4.3.3)
%     e = initialize_terms()
%     run_carpentry_compiler()
%     crossover_and_mutate()
%     select_terms() // selects Npop terms from 2 Npop terms
%     ....
% \end{lstlisting}

% N_pop is the population size.


 
% \begin{algorithm}[htb]
%   \caption{Iterative Contraction and Extension of BOP E-graphs.}
%   \label{alg:Framework}
%   \begin{algorithmic}[1]
%     \Require
%       A feasible design space, $\mathcal{D}$; an initialized BOP \Egraph encoding $K_d$ design variations, each with $K_f$ \afabvars;
%       %Performance measurement of each E-class $P_{e-class}$; 
%     \Ensure
%       Pareto front including (design, fabrication) pairs;
%     \State Extract Pareto front (\autoref{subsec:extract});
%         \begin{itemize}
%             \item Initialize $N_{pop}$ terms; %note...
%             \item Evaluate each term with a local Carpentry Compiler;%Note the different;just one layer
%             \item Term crossover and mutation;
%             \item Select $N_{pop}$ terms from $2 \times N_{pop}$ terms; 
%             \item Goto the second step if the 2 terminal criteria do not meet;% NSGA-III generalized
%         \end{itemize}
%     \label{code:fram:extraction}
%     \State BOP \Egraph Contraction (\autoref{subsec:constraction});
%         \begin{itemize}
%             \item Update $U_{score}$ and $E_{score}$ of each \eclass; 
%             \item Compute the pruning score $P_{score}$ of each \eclass;
%             \item Pruning the \eclass when its $P_{score} \leq P_{rate}$; 
%         \end{itemize}
%     \label{code:fram:pruning}
%     \State BOP \Egraph Extension (\autoref{subsec:extension}), goto ~\ref{code:fram:extraction};
%         \begin{itemize}
%             \item Generate $K_d$ new design variations (\autoref{subsec:des-var});
%             \item Include more \afabvars with the \fabheur algorithm (\autoref{subsec:fabheur});
%         \end{itemize}
%     \label{code:fram:more-designs} 
%     \State Goto ~\ref{code:fram:extraction} if the 2 terminal criteria do not meet;
%     \label{code:fram:termination} 
%     %Goto ~\ref{code:fram:extraction} if the 2 terminal criteria do not meet;
%   \end{algorithmic}
% \end{algorithm}

==> algorithm.tex <==
% \chandra{Sorry if this is too early for this comment, but eventually
% I would want to see the grammar for your DSL.
% Do you have a single DSL that represents both designs and the fabrication
% plans?}


\section{Optimization Algorithm}



%recall our goal, challenges, and key idea 


%The key observation is that we can take advantage of rampant sharing. Sharing between different design variations is possible because they may use the same set of parts. Furthermore, a set of parts can be fabricated with some specific fabrication process. When exploring and optimizing fabrication plans for a design variation, it might be useful to identify all the fabrication processes that will manufacture the set of parts it uses. This concern ultimately results in the fine-grain sharing of fabrication processes between \amy{the fabrication plans of} multiple design variations, and reinforces the utility of sharing sets of parts. \amy{Something about this was kind of confusing... So sets of parts = eclasses, and fabrication process = enodes. But it doesn't seem like there's a clear relationship between those two. Where is the bridge between sets of parts and fabrication processes? I feel like we should be building towards a point that the user can make their own intuition for how the bop e-graph is set up. I reworked it to try to bridge it but not sure if it's still right/what was initially intended.} Because searching for full \fabplans is difficult, we could first search for possible \fabplans for a sub-set of parts. Then these sub-set \fabplans can be used to compose the full \fabplans. Based on this observation, our insight is that a hierarchical data structure which could encode the \fabplans for sub-set of parts could be useful for encoding a large number of design variations and their possible \fabplans in an compact manner.

%E-graphs, commonly-used in the programming languages domain, are a perfect fit. Recently, several works have applied E-graph in to CAD/CAM domain. In this paper, we propose a new type of E-graph and a new extraction technique used to solve this design and fabrication joint optimization problem. This section will first give the definition of our proposed BOP E-graph. Then, we describe the output from our search framework. After that, a brief overview of our algorithm is given. \adriana{Some of this can go in the intro}


\subsection{Algorithm Overview}
\label{sec:algorithm-overview}



%As shown in Algorithm 1, we propose \textbf{Iterative Contraction and Extension on E-graphs (ICEE)} to search for the Pareto front pairs of design and their \fabplans. In the initialization step, two tasks are desired to work out. First, we need to detect all geometric joints and enumerate all candidate connecting variations for each joints. With different joint connecting variations, different design variation could be generated, as shown in Figure~\ref{fig:joints}. 
%Second, an initialized BOP E-graph need to be built starting from randomly selecting a set of design variations. For these design variation, we build an initialized BOP E-graph by applying an heuristic packing-driven e-graph construction procedure proposed in ~\cite{wu2019carpentry}. The key idea of heuristic packing-driven e-graph construction is that...

%The initialized BOP E-graph is not supposed to encode the global optimal \fabplans for the initialized design variations. However, we could extract the Pareto front \fabplans so far from the current BOP E-graph. We apply an genetic algorithm based on non-dominated sorting technique to extract the Pareto fronts for the current design variations. After the first extraction procedure, we could rank all of the design variations based on their current fabrication objectives. Some new design variations could be generated based on the existing design variations by a joint encoding based crossover and mutation operations. Before including these new generated design variations into the BOP E-graph, a pruning operator and an extending operator are applied to the current BOP E-graph. Our intuition is to prune a set of e-classes and e-nodes which have low contributions to the current Pareto front \fabplans. With the pruning operation, we suppose to keep the size of the e-graph manage-able in which only a good candidates are survived in the BOP E-graph. And the extending operator is used to explore more equivalent variations from some good candidate e-classes and e-nodes. We propose two key measurements to select the pruning and extending e-classes, the exploration score and utilization score which will be described in detail in the following section. With these new generated design variations, the BOP e-graph can be updated with the heuristic packing-driven e-graph construction procedure. Indeed, the whole searching process follows a loop between contraction extraction stages. With such procedure, the BOP E-graph will try to cover the Pareto optimal design and fabrication searching space without covering the whole combinations space.  




%Rough to fine objective estimation

Step 1: Initialization:
1.1 Init K/4 terms;
1.2 Evaluate each term by computing its cutting order with CC;


Step 2: Generate  K new terms by crossover and mutation
	*Note the difference that for cross-over before we would randomly select a common e-class and do the flip there.
*If there is NO e-class that is the same and in this case we will simply pick one of the parents at random and just do mutation. 
*The crossover works over terms from different designs;

Step 3: Evaluate new terms generated from Step 2;

Step 4: Select K terms from the 2K terms; Go to Step2. 
Note: Since cutting order is slow, a rough to fine process can be used. First apply several iterations with rough estimation to remove the really bad terms.
Note: the e-graph is fixed, we do no changes, we only do extraction. 
Note: For all of the Designs and Fabrication plans that are currently represented in the e-graph, this algorithm finds the ones in the pareto front. 


\subsection{Design Variations}
We simply run crossover and mutation on the parent designs that are “doing well” - how to choose the parents? Right now we choose the parent that are on the current pareto front. We can think more about how to choose these parent later. We may want to consider different metrics and we may also want to add some more randomization later. But it’s fine for now. (we have something working, we may want to tweak it later but let’s focus on the other problems now so we have something end-to-end). 
(MCMC?)(Distribution learning...)

\subsection{Fabrication Variations}

4.1 For the new designs, we extend BOP E-graph as Step 1.2. This step will include new e-classes and fab e-nodes;

4.2 Select a few e-classes (from any design and at any level) and we create more packing variations for them. -> improve the whole quality of the current e-graph. How do we do this?
Choose which e-class. Life time + choose some at random too. 
How do we generate new packing. DAI can be used for this. 


Note: these might also need iteration. We may want to come back and think of other ideas for choosing e-classes later but this is good for now.  

\subsection{Pruning}

\begin{itemize}
    \item exploration score
    \item utilization score
\end{itemize}


==> results.tex <==
% \begin{table}[]
% \scriptsize
%     \centering
%     \begin{tabular}{l||r|r|r|r||r|r||r|r|r|r}
%     \multicolumn{1}{c}{} 
%     & \multicolumn{4}{c}{Model Statistics} 
%     & \multicolumn{2}{c}{Parameters} 
%     & \multicolumn{4}{c}{Params derived from $\alpha$ and $\beta$} \\
%     Model & \#P & \#J & \#JV & \#DV              & $\alpha$ & $\beta$ & $K_d$ & $K_f$ & $K_m$ & $N_{pop}$
% \\ \hline  Frame        & 4  & 4  & 22 & 13      & 1    & 1  & 4  & 8   & 4   & 8   
% \\ \hline  Long frame   & 6  & 8  & 16 & 65      & 2    & 2 & 8  & 32  & 8   & 48  
% \\ \hline  Art window   & 12 & 13 & 28 & 18272   & 1    & 1 & 32 & 64  & 10  & 128 
% \\ \hline  Art bookcase & 12 & 6  & 16 & 192     & 1    & 10 & 8  & 160 & 6   & 32  
% \\ \hline  Chair        & 14 & 14 & 32 & 66438   & 1    & 1  & 32 & 64  & 10  & 128 
% \\ \hline  Table        & 12 & 8  & 23 & 1140    & 1    & 1  & 16 & 32  & 8   & 64  
% \\ \hline  Frame cube   & 12 & 8  & 23 & 5       & 4    & 1  & 8  & 16  & 8   & 128 
% %\\ \hline  Window\_1    & 12 & 16 & 40 & 1520052 & 0.25 & 1 & 32 & 64  & 3.5 & 32  
% \\ \hline  Window    & 12 & 16 & 32 & 10463   & 1    & 1          & 32 & 64  & 10  & 128 

%     \end{tabular}
%     \caption{Statistics for each input model, showing the complexity with the number of parts ($\#P$), joints ($\#J$), joint variations ($\#JV$), design variations that define unique bag of parts ($\#DV$). We also show tuning parameters $\alpha$ and $\beta$ used for every experiment. The resulting parameters used in ICEE, which are computed as a function of the model statistics and the tuning parameters. }
%     \label{tab:modelstats}
% \end{table}

\begin{table}[]
\scriptsize
    \centering
    \begin{tabular}{l|c|c||c|c||c|c|c|c}
    \multicolumn{1}{c}{} 
    & \multicolumn{2}{c}{Model Statistics} 
    & \multicolumn{2}{c}{Parameters} 
    & \multicolumn{4}{c}{Params derived from $\alpha$ and $\beta$} \\
    Model & \#P &  $\nd$       & $\alpha$ & $\beta$ & $K_d$ & $K_f$ & $K_m$ & $N_{pop}$
\\ \hline  Frame        & 4   & 13      & 1    & 1  & 4  & 8   & 4   & 8   
\\ \hline  Long frame   & 6   & 65      & 2    & 2 & 8  & 32  & 8   & 48  
\\ \hline  Art window   & 12  & 18272   & 1    & 1 & 32 & 64  & 10  & 128 
\\ \hline  Art bookcase & 12 & 192     & 1    & 10 & 8  & 160 & 6   & 32  
\\ \hline  Chair        & 14  & 66438   & 1    & 1  & 32 & 64  & 10  & 128 
\\ \hline  Table        & 12  & 1140    & 1    & 1  & 16 & 32  & 8   & 64  
\\ \hline  Frame cube   & 12  & 5       & 4    & 1  & 8  & 16  & 8   & 128 
%\\ \hline  Window\_1    & 12 & 16 & 40 & 1520052 & 0.25 & 1 & 32 & 64  & 3.5 & 32  
\\ \hline  Window    & 12  & 10463   & 1    & 1          & 32 & 64  & 10  & 128 

    \end{tabular}
    \caption{Statistics for each input model, showing the complexity in number of parts ($\#P$) and number design variations that define unique bag of parts $\mathcal{D}$. We also show tuning parameters $\alpha$ and $\beta$ used for every experiment and the resulting parameters used in ICEE, which are computed as a function of the model statistics and the tuning parameters. }
    \label{tab:modelstats}
\end{table}








\section{Results and Discussion}
\label{sec:results}

In order to gauge the utility of our tool, we want to answer the following questions:
\begin{enumerate}
% \chandra{\item Does the additional exploration of the design space
% enable us to find better fabrication plans that either have different trade offs or are more interesting or outperforms the previous approach.

% \item how does our result compare against expert results?

% \item how does our approach 
% }
    \item How much does searching the design space with the fabrication space improve generated \fabplans?
    \item How does our tool compare with domain experts who are asked to consider different design variations?
    \item How does our tool's performance compare to a baseline na{\"i}ve approach?
    % other carpentry optimization tools?
    % \item How do our algorithmic contributions affect performance?
\end{enumerate}


%introduce models; two tables; running environment;
We evaluate our method using the examples in \autoref{fig:models}. 
Statistics for each model are shown in Table~\ref{tab:modelstats}. 
In our experiments, the parameters used in our ICEE algorithm are scaled based on the complexity of each model, measured in terms the number of parts $n_p$ and the size of the design space $\nd$. We also exposed a set of tuning parameters $\alpha$ and $\beta$. While these are set to the default value of $1$ for most experiments, these parameters allow us to tune how much computations is spent on design vs fabrication plan exploration. For example, in complex models where the joint angles vary freely, we typically require more exploration of the space of fabrication plans to find solutions. The number of initialized design variations $K_d$ is set to $K_d = \alpha \times 2^{\lceil { \log_{10} \nd }\rceil}$. For each design variation, encodes $K_f$ \afabvars to the \bope, $K_f = \beta \times 2^{\lceil { \log_{10} \nd }\rceil + 1}$. During the design variation generation step, $K_m$ is set to $ K_m = 2 \alpha \times \lceil { \log_{10} \nd }\rceil$. In the Pareto front extraction step, the population size $N_{pop}$ is set based on the number of parts, $n_{p}$, of a canonical design and $\nd$, $N_{pop} = \alpha \times  {\lceil {\log_{2} n_{p}} \rceil} \times 2^{\lceil { \log_{10} \nd }\rceil}$. %$\alpha$ and $\beta$ are two scaling parameters whose default value is $1$. $\alpha$ and $\beta$ for each model is shown in~\autoref{tab:modelstats}. 
%\haisen{Review will ask why we use different $\alpha$ and  $\beta$?} \adriana{I agree this is super messy. Do you really need to cherry pick this? I was hoping you would use this for testing purposes only.}
%All of these parameters could also be set by users manually.
%For an input design $d_{input}$, we could calculate the number of all possible design variations $N_{\mathcal{D}}$ of $d_{input}$ with the product the connecting variations of each joint.



We report the running times of our algorithm in \autoref{tab:runningstats} for the list of models in \autoref{fig:models}.
The above times are measured on a desktop computer with 32GB RAM and a 3.5 GHz 6-Core Intel Core i7 CPU.

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/models-flat-no-2d.png}
    \caption{Models used for all experiments in \autoref{sec:results}.}
    \label{fig:models}
\end{figure}



\begin{table}[h]
\footnotesize
    \centering
    \begin{tabular}{c|rrrrrrr}
    Model & \#Iter & \#EDV & \#Arr & \#PDV & CEt(m) & Et(m) & Total(m)  \\
    \hline
Frame        & 22 & 11  & 343    & 3 & 0.9   & 0.7   & 1.6   \\
Long frame   & 31 & 52  & 16034  & 3 & 9.2   & 5.1   & 14.3  \\
Art window   & 41 & 190 & 28244  & 8 & 152.5 & 207.7 & 360.1 \\
Art bookcase & 31 & 18  & 98617  & 3 & 16.0  & 57.0  & 73.0  \\
Chair        & 55 & 57  & 342014 & 7 & 77.4  & 26.3  & 103.8 \\
Table        & 36 & 75  & 52632  & 7 & 18.8  & 21.2  & 40.0  \\
Frame cube   & 37 & 5   & 14958  & 4 & 6.3   & 3.4   & 9.8   \\
%Window\_1    & 57 & 725 & 264362 & 1 & 167.0 & 149.7 & 316.7 \\
Window    & 52 & 354 & 794614 & 3 & 165.2 & 78.9  & 244.2
    \end{tabular}
    \caption{
    %Pipeline running time and performance for each testing model. This table shows algorithm running time taken in each stage, 
    %the number of explored design variations, the number of explored e-classes/e-nodes, the final hypervolume.
Some statistics and running times for our ICEE algorithm. We report the number of iterations (\#Iter), explored design variations (\#EDV) and arrangements (\#Arr), and Pareto front design variations (\#PDV).
We report the running time of \bope contraction and expansion (CEt), and Pareto front extraction (Et), as well as the total time. All running time are in minutes.}
    \label{tab:runningstats}
\end{table}



\subsection{Benefits of Design Exploration}
%  For each example, we compute the Pareto front generated by our program with design variations and \fabplan variants and the Pareto front generated considering \fabplan optimization only. 
%  These are compared with the Pareto front of the initial design. \adriana{this was wu et al.}
%  This comparison is of particular interest as our contributions --- the 
%  the BOP E-graph capable of representing different design variations, and ICEE 
%  --- are only relevant if exploring more designs truly improves fabrication cost.
 
 
\begin{figure*}
    \centering
    %\includegraphics[width = \linewidth]{images/comparison-no-design-opt.png}
    \includegraphics[width = \linewidth]{images/result-pareto.pdf}
    \caption{Pareto fronts computed from our pipeline with design optimization as colored dots. Each color corresponds to a different design. These are compared against Pareto fronts computed without design optimization (fabrication optimization only, using the original model as the input design) as squares, and expert fabrication plans as diamonds. Often, fabrication plans from a design variant are more optimal than those generated from an input design.}
    \label{fig:comparison-design-optimization}
\end{figure*}


\begin{figure}
    \centering
    %\includegraphics[width = \linewidth]{images/comparison-no-design-opt-fab.png}
    \includegraphics[width = \linewidth]{images/artwindow-2.pdf}
    \caption{
    Three fabrication plans from the Pareto front of the Art Window and
    the designs from which they are generated. 
    Plans 1, 2, and 3 are the lowest-cost plans from the front with respect to material cost, precision, and time respectively. 
    Plan 1 uses a few long pieces of stock for all parts, which fit because each angled part is short enough to be packed onto a single 96x2x2. This plan also packs very carefully, producing very minimal leftover stock (contrast plans 2 and 3).
    Plan 2 maximizes precision by choosing the best reference points for each angled cut, regardless of whether it is economical in time or material.
    Plan 3 has the lowest time cost. Notice that we make all cuts with the same angle before making cuts with a different angle, minimizing setups. Also, in this design, we retain the three long identical pieces that zigzag across the interior of the window, which correspond to the parts in the bottom three pieces of lumber. For identical cuts, we stack stock so that one cut can be applied to several pieces of stock.
    % Flexibility in the design space corresponds to a wider diversity and more varied selection of plans.
    }
    \label{fig:comparison-design-optimization-fab}
\end{figure}

To demonstrate the benefit of simultaneous exploration of the design variation 
 and fabrication plan spaces, 
 we compare our tool against 
 optimizing the fabrication plan for a single design. 

\autoref{fig:comparison-design-optimization}
 shows the comparison between our pipeline and the Carpentry Compiler pipeline~\cite{wu2019carpentry}
 which only considers a single design. We explore the trade-offs for fabrication time and material usage for the designs where all cuts can be executed with standard setups (these are considered to have infinite precision) and include a third objective of precision error for the models where that is not possible.  
The Pareto fronts across designs generated by our tool covers a larger space and 
 many of our solutions dominate those from previous work. 
 %\adriana{This is true for the 2D plots for sure. TODO: for the 3D plots check if there is any solution that is on CC that dominates and if so report. If not, complete previous sentence with ",while non of the solution from the previous work dominate our solutions". After you're done, delte my comment!}
\autoref{fig:comparison-design-optimization-fab} shows some fabrication plans generated by our tool.

%Table ~\ref{tab:runningstats} shows the running time it took for each model shown in Figure ~\ref{fig:models}.

%For each model you have the Pareto front of the initial design (cc result), and the Pareto front that you get with you technique. (maybe some of this data will be in supplemental and we will report here in a summary). 

%We run the carpentry compiler for one design and compare to ours in terms of quality and time. Maybe in some cases we can even do better time! :) 


\subsection{Comparison with Experts}
% \begin{table}
%     \centering
%     \begin{tabular}{c|cccc}
%     Model & Variant & Score & Min. to gen (expert) \\
%     \hline
% Frame      & 1 & 4 & 30 \\
% Frame      & 2 & 4 & 60 \\
% LongFrame  & 1 & 4 & 45 \\
% Window     & 1 & 4 & 30 \\
% Bookcase   & 1 & 4 & 30 \\
% Cube       & 1 & 4 & 60 \\
% Cube       & 2 & 4 & 75 \\
% 2DBookcase & 1 & 4 & 180 \\
% Dresser    & 1 & 4 & 100
%     \end{tabular}
%     \caption{Data for expert \fabplans.\haisen{remove this table maybe. We have illustrated the expert result in figure 7. For the design time, we could report the average time.?}}
%     \label{tab:expert-table}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{images/expertPlans-PLACEHOLDER.png}
%     \caption{The optimal \fabplans for different projects, as generated by experts.}
%     \label{fig:expert-results}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{images/expertVsPareto-PLACEHOLDER.png}
%     \caption{Comparing each optimal \fabplan to our pareto front, computed over joint design and fabrication variations}
%     \label{fig:expert-vs-pareto}
% \end{figure}


% We want to know if our tool can produce results that are at least as good as expert \fabplans, if not better.Experts are the current state-of-the-art for creating design variations and their optimal \fabplans.

For each model, we asked carpentry experts to generate design variations and \fabplans.
The resulting points are plotted as diamonds in \autoref{fig:comparison-design-optimization}.
Since experts produce each solution by hand,
 they produced Pareto fronts with many fewer solutions than our tool.
Solutions generated by our tool dominate the expert solutions on every model. 
%\adriana{Confirm this is true and then delete my comment.}
This suggests that, although expert plans seem sensible,
 our tool generates better output thanks to its 
 ability to generate more design variations and \fabplans, 
 including potentially unintuitive packing or cutting orders,
 and evaluate them much more quickly than a human.
%\amy{Common features of expert designs - modularity (smaller pieces of lumber), symmetry - key insights}

% Figure \ref{fig:expert-results} shows the resulting designs, as well as the associated cost of each 
% packing and cutting order.

% Because there are not enough points, 
% we are unable to generate a Pareto front for the experts' plans 
% --- an inherent advantage present in the programmatic approach.
% Instead, we juxtapose the output of each method. 

% Looking at the results in Figure \ref{fig:comparison-design-optimization},
% our algorithm finds points on the Pareto front 
% that dominates the experts' for every model.
% This is because, although expert plans seem sensible,
% we are able to generate more design variations and \fabplans, 
% including potentially unintuitive packing or cutting orders,
% and evaluate them much more quickly than a human.
% \amy{Common features of expert designs - modularity (smaller pieces of lumber), symmetry - key insights}

% \amy{Optimizing cutting order is REALLY tedious for humans! Need to evaluate all possible reference points, and for angles, that might mean taking the time cost of setting up a different angle. But is that better than taking the precision loss across all n cuts? Also, expert \fabplans didn't vary that much/not very radical}


% Additionally, our tool is considerably faster than the human experts, 
% who on average spent 75 minutes creating their design variations.  
% Overall, we are able to achieve equivalent optimization without the knowledge of a domain expert,
% and much faster. Full detail of the expert plans is available in \autoref{tab:expert-table}. \adriana{How much of this time is spent actually designing? I'm not sure we can claim performance... but maybe... We may need to look a the results for this but what I'd like to say is: in all experiments we found solutions that have different trade-offs in x out of the y experiments we found solutions that dominate the experts designs (i.e. they are better in every metric). Again point to supplemental for all results and add the key ones here.}




\subsection{Performance Evaluation}
\label{subsec:perf-eval}
% Why do we care about brute force? What are we trying to show?

To test whether the \bope's sharing is important for our tool's performance,
 we compare against a nested-optimization pipeline built on the Carpentry Compiler~\cite{wu2019carpentry}.
The baseline approach invokes the Carpentry Compiler pipeline on
 each design variant that our tool explores,
 and then it takes the Pareto front across all design variations. 

\begin{table}
\footnotesize
    \centering
    \begin{tabular}{crr|rr|rr}
     \multirow{2}{*}{Model} & \multirow{2}{*}{$\nd$} & \multirow{2}{*}{\#EDV} & \multicolumn{2}{c}{Time (min)} &  \multicolumn{2}{c}{Hypervolume} \\
    \cline{4-7}
     &  & & Ours & Baseline & Ours & Baseline \\
    \hline
{Frame}       & 13& 11  & 1.6 & 5.4 & 971739& 971739 \\
{Long frame}  & 65& 52 & 14.4 & 120.4  & 957083 & 957083\\
{Table}  & 1140& 75 & 40.0 & 684.7  &962324& 962320\\
{Window}  & 10463 & 354 & 244.2 & $^{\star}$2124.0 & 955533 & -
    \end{tabular}
    \caption{
    Results of the performance validation experiment.
    ``Ours'' indicates the ICEE algorithm of this paper. 
    ``Baseline'' indicates extracting the Pareto front \fabplans for each design variation explored by our method independently with the Carpentry Compiler pipeline~\cite{wu2019carpentry}. 
    The size of design space $\nd$ and the number of explored design variations (EDV) are also reported.
    $^\star$This model's running time under the baseline scheme
     is estimated from the running time of a subset of the 354 explored design variations.
     Hypervolume cannot be estimated from this subset.
}\label{tab:time-comparison}
\end{table}

 
We choose four models of varying complexity to evaluate performance and show results in \autoref{tab:time-comparison}.
For the models which the baseline method with no sharing was able to run to completion,
 the hypervolume is nearly identical.
This indicates that our co-optimization approach yields similar results to the nested approach over the same space.
When it comes to performance, 
 our approach is about one order of magnitude faster.
We attribute this speedup to the sharing captured by the \bope;
 we only had to evaluate common sub-designs and sub-fabrication-plans one time,
 whereas the baseline shared no work across its different invocations for each design variant.
% As a baseline, we first compare our implementation with a brute-force search approach.


% \chandra{explain what the two experiments are in Table 4}
% The space of possible \fabplans grows exponentially, so brute force 
% is tractable only for designs A and B, shown in Figure ~\ref{fig:comparison-brute-force}; we estimate the brute force runtime for all other designs.

% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{images/comparison-brute-force.png}
%     \caption{Comparison results between our methods and brute force method. The brute force methods mean that we randomly select a set of design variations. For each variation, we run Carpentry Compiler pipeline to generate its Pareto fronts \fabplans. Then we compare the two methods with running time and performance indicated with hypervolume metherrics. There is only two simple, frame and long frames which are tractable with the brute force method.}
%     \label{fig:comparison-brute-force}
% \end{figure}


% In order to assess the quality of our tool's \fabplans, we use the hypervolume measure, where a larger hypervolume implies more optimal results.
% maybe there's a better mathematical way to express this?
% like closed neighborhood on the two points being compared

% \amy{I found the following two paragraphs but they are the same... Also, we talk about time to run brute force here, and it should really below in the below paragraph}
% Figure \ref{fig:comparison-brute-force} indicates that for each design, our approach 
% always beats out the brute force approach, and it reaches
% the higher hypervolume much faster.

% We also find that the hypervolume of the brute force approach is always equal to or less than that of our approach. Although we are using only a subset of design variations, the evidence suggests that ICEE approaches optimality. \amy{Maybe we could be stronger about this... or less strong, depending.}

% \adriana{we also talked about the performance evaluation with taking the k designs that we end up exploring and comparing testings just those, the "Max" idea.}



% Why?
%Our tool has many obvious advantages over brute force.
% Complete enumeration is very expensive,
% and so the brute force method may not be able to 
% discover the optimizations that our method ultimately
% used in the final \fabplan. 

% \paragraph{Estimating brute force performance.}
% To estimate how long it might have taken a complete brute force solution, 
% we measure the runtime of brute force methods on a subset $S$ of possible design variations $D$, then multiply that number by $\frac{\mid D \mid}{\mid S \mid}$ to find approximately how long it would take to optimize over all design variations. 

% \amy{Need some performance comparison results}

\subsubsection{Performance Analysis}

% The following ARE real numbers! 
On average, our pipeline spends 30.1\% of its runtime in design extraction, 18.9\% of its time generating packings, 28.9\% of its time assigning cutting orders, and 13.4\% of its time in applying genetic algorithms. This translates to 48.9\% of its runtime in the expansion and contraction phase, 42.3\% in the extraction phase, and the other 8.8\% everywhere else. Concrete runtime numbers are available in Table \ref{tab:runningstats}.

 \begin{figure}[h!]
\centering
\includegraphics[width= \linewidth]{images/hv-vs-time.pdf}
\caption{
 Hypervolume of the Pareto front as a function of running time.
% This figure depicts what percentage of the hypervolume was achieved at different points during the execution of our tool.
% In general, the hypervolume jumps quickly each iteration to converge upon the hypervolume early to midway through.
The average time to reach the final hypervolume is 56.8\% of total runtime; the min and max time are 15.1\% and 86.1\%.
The average, min, and max times to reach 99\% of the final hypervolume are, 20.0\%, 5.5\%, and 83.5\% of the total runtime.
Complex models with more variations, like the Art window and Art bookcase,
 take longer to reach close to a final hypervolume compared to simpler models like Long frame
 since their design space is much larger.
}\label{fig:time-quality}
\vspace{-2mm}
\end{figure}



\autoref{fig:time-quality} shows how our algorithm converges,
 i.e., how the hypervolume of the Pareto front increases over time.
%\max{I don't think we need to say much else here. It's just data.}

% We also want to know how long it takes to produce a Pareto front 
%  whose hypervolume exceeds some threshold, i.e. when the 
%  line in \autoref{fig:time-quality} tapers off.
%  20 iterations of the hypervolume not changing, so we might want to change
%  the below discussion based on this info.}
% Here, we choose the time that it takes to reach 99\% of the final hypervolume.
% Though results vary somewhat by the input model, we find that in general
% we reach the hypervolume after not much time has elapsed. Encouragingly, this also suggests
% that we converge upon a hypervolume reasonably soon, and that the hypervolume does not grow 
% forever using our method. \amy{Need to check this conclusion over}
% The fact that we don't immediately always reach the final hypervolume also suggests that the solution isn't entirely trivial.

% \paragraph{Impact of sharing} \amy{Discuss table 2 here}

\subsection{Fabricated Results}

We validated our pipeline by physically constructing some of the models 
 according to the design variation-fabrication plan pairs generated by our tool.
\autoref{fig:fabrication-result} shows the results.
% that our pipeline generated by exploring the joint design and fabrication space.  \autoref{fig:fabrication-result}. Fabricated results for the chair are also highlighted in the teaser image, Figure~\ref{fig:teaser}. 



\begin{figure}[h!]
    \centering
    %\includegraphics[width = \linewidth]{images/fabrication-result.png}
    \includegraphics[width = \linewidth]{images/manufactured.png}
    \caption{Fabrication results of two window variations. The different design and fabrication plans trade off fabrication time and material usage.}
    \label{fig:fabrication-result}
\end{figure}




\subsection{Limitations and Future Work}
\label{subsec:lim}
%\chandra{remove tilted window from fig 6, just describe the tilted
%window here in the text}
Our approach does not
 guarantee an exhaustive
 exploration of the design space in general.
Consider the design of the
 ``Window''
 in \autoref{fig:models}.
If we permit
 this model to have  angled
 joints instead of just 90 degree joints, 
 the space of design variants becomes much larger.
 %Window 1 (\autoref{tab:modelstats})
% (the variants for Window 2 are in fact a subset of the
% variants for Window 1).
Ideally, the result for this new window variant should be at least as
 optimal as the result for the original window.
However, our approach was able to explore only a
 portion of the vast design space ($\nd=1520052$, compared to $\nd=10463$ for the simpler window model) and found a worse landscape of solutions (\autoref{fig:lim}).
For models with a large design space,
 if the initial design variants picked by our
 algorithm are too far
 from the optimal ones,
 then our algorithm
 may never reach those optimal points.
 
\begin{figure}[h!]
    \centering
    \includegraphics[width = .7\linewidth]{images/limitations.pdf}
    \caption{Example showing a limitation of our approach:
    allowing the Window model to have arbitrarily angled joints
    makes the search space of design variants too large for
    our approach to fully explore.
    Our approach found only 2 Pareto-optimal results for this new window
    (Window 2)
    whereas it found 3 for the original model (Window 1)
    which only allowed 90$^{\circ}$ joints.}
    \label{fig:lim}
\end{figure}
Our current approach encodes only discrete design
 variants in the \bope.
An interesting direction for future work would be to
  support continuous variations in the designs space
  which can provide a larger space of fabrication plans
  to explore.
However, supporting continuous design variants in an \egraph
 would require designing a new metric for comparing two
 design variants for equivalence.
This is challenging because e-graphs
 heavily exploit transitivity,
 so any error in the metric
 could lead to arbitrarily different designs being
 considered ``equivalent''.
% A metric like Hausdorff distance that works
%  well for discrete variations will no longer work.
 
Several steps of our algorithm can
  also be parallelized for performance
  (e.g. generating design variants)---we leave this
  as an extension for the future.

We are also keen to explore broader applications of the
  ICEE strategy for integrating feedback-directed search
  in other \egraph-based optimization techniques.
Past work applying \egraphs for design optimization
  in CAD~\cite{szalinski} and for
  improving accuracy in floating-point code~\cite{herbie}
  have relied on ad hoc techniques for controlling the
  growth of the \egraph, e.g., by carefully tuning
  rules used during rewrite-based optimization.
We hope to explore whether ICEE can help
  with optimization in such domains by
  focusing the search on more-profitable candidates
  and easing implementation effort by reducing the
  need for experts to carefully tune rewrite rules.

Another direction we are eager to explore is
  accounting for other factors in the Pareto front.
Currently, our technique finds a
 design variant and fabrication plan
 that optimizes fabrication time,
 material cost, and
 precision.
Other interesting factors that can guide the
 search include ease of assembly,
 stability, and strength of the part.

% Limitations and future work:
% \chandra{1. key limitation is that we cannot guarantee that we will fully explore the space. in particular, if the space is too large and there is one design that achieves optimality, and we start from one that is far from it, we may not get to that good design. e.g. window 1.

% 2. our search space did not contain continuous variations. Good for FW. We could try to parallelize some parts of the implementation,

% 3. a. assembly: we also did not consider other cost metrics like assembly.
%   b. minimized fab cost, but since we are exploring a joint design and fab space, we could consider
% stability, strength, performance etc.

% }

% \begin{itemize}
%     \item window 1 example
%     \item Do not support free-form objects;
%     \item No guarantees of convergence;
%     \item Our current BOP E-graph could only encode discrete parameters. 
%     Did not consider continuous variations; Figure ~\ref{fig:continuous-variation} shows one example that reduce the fabrication cost with tuning the continuous parameters of the input feasible design. 
%     \item We apply the objective evaluation method in Carpentry Compiler which may not accuracy;
%     \item Only consider subtractive approaches without additive process. We did not consider to merge multiple parts into one single part.
%     \item Our framework could not guarantee to find better design variations than input design. For some models, we could not find any design variations whose fabrication cost is lower than that of the original design. For example XXX, the input model only use two kinds of parts. With our current evaluation method of fabrication cost, it tends to generate lower cost fabrication plans with less number of part types. 
%     \item FW: Many steps in our algorithm can be parallel. In our current implementation, we did not do that.
%     \item FW: We did not consider approximated part fabrication. During fabrication, if a part is almost what we want, we could just take it. Maybe we could save more material time and cost. Our current pipeline only consider small modification of design. During fabrication, we could also allow some fabricaiton error to improve cost further.   \item We did not consider approximated part fabrication. During fabrication, if a part is almost what we want, we could just take it. Maybe we could save more material time and cost. Our current pipeline only consider small modification of design. During fabrication, we could also allow some fabricaiton error to improve cost further.
   
% \end{itemize}


% Future work:
% \begin{itemize}
%     \item Future work: Assembly - take into account how assembly will happen when optimizing the design - make it easy to assemble and also structure stability. 
%     \item Future work: Stability - different joint variations will affect the design stability. One interesting future work is to include stability measurement into our pipeline. We prefer to output structure-sound design variations with lower fabrication cost.
%     \item Future work: include both continuous and joint variations to our framework.
%     \item Extend the key idea of our pipeline to other domains. We only demonstrate our design and fabrication jointly encoding and optimization in carpentry domain. It's interesting to extend the idea to other fabrication process, such as additive which also involve a large design space and a multiple stage planning problems.
    
%     \item We don't consider strength of the part in the
%     pareto front. The chair is a good example
%     of this---the one we pick may not be the strongest.
%     \item consider branch and bound technique for multi-objective
%     \item improve our current low-bound computation method
    
% \end{itemize}

==> results_old.tex <==
\begin{table}
    \centering
    \begin{tabular}{l||r|r|r|r|r} \hline
    model & \#P & \#J & \#JV & \#DV & \#UDV 
\\ \hline  frame        & 4  & 4  & 22 & 81      & 13      
\\ \hline  long frame   & 6  & 8  & 16 & 256     & 65      
\\ \hline  art window   & 12 & 13 & 28 & 18432   & 18272   
\\ \hline  art bookcase & 12 & 6  & 16 & 288     & 192     
\\ \hline  2d bookcase  & 15 & 22 & 44 & 4194304 & 4194304 
\\ \hline  dresser      & 10 & 10 & 25 & 5760    & 5045    
\\ \hline  chair        & 14 & 14 & 32 & 82944   & 66438   
\\ \hline  cube frame   & 12 & 8  & 23 & 4374    & 5       
\\ \hline  window\_1    & 12 & 16 & 40 & 1679616 & 1520052 
\\ \hline  window\_2    & 12 & 16 & 32 & 65536   & 10463  
    \end{tabular}
    \caption{Statistics for each input model, showing the complexity with the number of parts ($\#P$), joints ($\#J$), joint variations ($\#JV$), design variations ($\#DV$) and unique
    design variations ($\#UDV$) without redundant (design redundant is illustrated in \autoref{fig:joints}).}
    \label{tab:modelstats}
\end{table}



\section{Results and Discussion}

%introduce models; two tables; running environment;
We will evaluate the performance of our method using the examples in Figure~\ref{fig:models}. Statistics for each model are shown in Table ~\ref{tab:modelstats} showing varying amount of parts and joint variations. We report running times of our algorithm in Table ~\ref{tab:runningstats} for the whole list of models in Figure ~\ref{fig:models}. The above times are measured on an Macbook Pro with 16GB RAM and a 2.3 GHz 8-Core Intel Core i9 processor.

%parameter setting
In our experiments, we set the same parameters for all models. Some parameters are scaled based on the complexity of each model, measured in terms of the size of the design space $\nd$. %For an input design $d_{input}$, we could calculate the number of all possible design variations $N_{\mathcal{D}}$ of $d_{input}$ with the product the connecting variations of each joint.
The number of initialized design variations $K_d$ is set to $K_d = 2^{\lceil { \log_{10} \nd }\rceil}$. For each design variation, the initialized BOP \Egraph encodes $K_f$ \afabvars, $K_f = 2^{\lceil { \log_{10} \nd }\rceil + 1}$. During the design variation generation step, $K_m$ is set to $ K_m = 2 \times \lceil { \log_{10} \nd }\rceil$. In the Pareto front extraction step, the population size $N_{pop}$ is set based on the number of parts, $n_{p}$, of a canonical design and $\nd$, $N_{pop} = {\lceil {\log_{2} n_{p}} \rceil} \times 2^{\lceil { \log_{10} \nd }\rceil}$. These parameters could also be set by users manually.

 
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/models-flat.png}
    \caption{Examples that will be used for all the experiments.}
    \label{fig:models}
\end{figure}



\begin{table}
    \centering
    \begin{tabular}{c|cccccc}
    model & Init(s) & Exploration(s) & \#designs & \#ec & \#en & HV \\
    \hline
Frame      & 4 & 4 & 12 & ? &  & ? \\
LongFrame  & 4 & 4 & 12 & ? &  & ? \\
Window     & 4 & 4 & 12 &   &  & ? \\
Bookcase   & 4 & 4 & 12 &   &  & ? \\
Cube       & 4 & 4 & 12 &   &  & ? \\
2DBookcase & 4 & 4 & 12 &   &  & ? \\
Dresser    & 4 & 4 & 12 &   &  & ?
    \end{tabular}
    \caption{Pipeline running time and performance for each testing model. This table shows algorithm running time taken in each stage, the number of explored design variations, the number of explored e-classes/e-nodes, the final hypervolume.}
    \label{tab:runningstats}
\end{table}

\subsection{Comparisons with Other Methods}
In order to gauge the utility of our tool, we want to answer the following questions with the evaluation.
\begin{enumerate}
    \item How much does searching the design space with the fabrication space improve generated \fabplans?
    \item Does our tool outperform domain experts who are asked to consider different design variations?
    \item How does our tool's performance compare to other carpentry optimization tools?
    \item How do our algorithmic contributions affect performance?
\end{enumerate}


\subsubsection{Comparison without Design Optimization}
 For each example, we compute the Pareto front generated by our program with design variations and \fabplan variants and the Pareto front generated considering \fabplan optimization only. 
 These are compared with the Pareto front of the initial design.
 This comparison is of particular interest as our contributions --- the 
 the BOP E-graph capable of representing different design variations, and ICEE 
 --- are only relevant if exploring more designs truly improves fabrication cost.
 
 
\begin{figure}
    \centering
    %\includegraphics[width = \linewidth]{images/comparison-no-design-opt.png}
    \includegraphics[width = \linewidth]{images/result-pareto.png}
    \caption{Pareto fronts computed from our pipeline with design optimization vs. Pareto fronts computed from Carpentry Compiler without design optimization. We show the comparison using the chair and window models.}
    \label{fig:comparison-design-optimization}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/comparison-no-design-opt-fab.png}
    \caption{The visualization results of some Pareto front points of the \fabplans in ~\ref{fig:comparison-design-optimization}. The first column shows one \fabplan visualization of the original design. The second and third columns give two fabrication  plan visualization of two design variations. Colors identify the process and
numbers the order of cuts. The costs are shown in the order: $f_c$, $f_p$, $f_t$ in square brackets below each figure.}
    \label{fig:comparison-design-optimization-fab}
\end{figure}

\begin{table}
    \centering
    \begin{tabular}{cc|cc|cc}
     \multirow{2}{*}{Model} & \multirow{2}{*}{Design} & \multicolumn{2}{c}{No Design Exp.} &  \multicolumn{2}{c}{With Design Exp.} \\
    \cline{3-6}
    \multicolumn{1}{c}{} & & Time & HV & Time & HV \\
    \hline
Frame      & id & 4 & 4 & 12 & ?  \\
LongFrame  & id & 4 & 4 & 12 & ?  \\
Window     & id & 4 & 4 & 12 & ?  \\
Bookcase   & id & 4 & 4 & 12 & ?  \\
Cube       & id & 4 & 4 & 12 & ?  \\
2DBookcase & id & 4 & 4 & 12 & ?  \\
Dresser    & id & 4 & 4 & 12 & ?
    \end{tabular}
    \caption{Time comparison with hypervolume}
    \label{tab:time-comparison}
\end{table}

Figures~\ref{fig:comparison-design-optimization} and~\ref{fig:teaser} shows the comparison between out pipeline (with design optimization) and the Carpentry Compiler pipeline~\cite{wu2019carpentry} (without design optimization). We could see that the Pareto fronts (indicating with larger colored dots) with design optimization cover much larger area in the performance space and the Pareto front points (indicating with smaller colored dots) computed from Carpentry Compiler are all dominated. Some Pareto front points are visualized in Figure ~\ref{fig:comparison-design-optimization-fab}. \adriana{added ref to teaser as well. Refer to sup material for the rest of the models. }

%Table ~\ref{tab:runningstats} shows the running time it took for each model shown in Figure ~\ref{fig:models}.

%For each model you have the Pareto front of the initial design (cc result), and the Pareto front that you get with you technique. (maybe some of this data will be in supplemental and we will report here in a summary). 

%We run the carpentry compiler for one design and compare to ours in terms of quality and time. Maybe in some cases we can even do better time! :) 

\subsubsection{Comparison with Experts}
\begin{table}
    \centering
    \begin{tabular}{c|cccc}
    Model & Variant & Score & Min. to gen (expert) \\
    \hline
Frame      & 1 & 4 & 30 \\
Frame      & 2 & 4 & 60 \\
LongFrame  & 1 & 4 & 45 \\
Window     & 1 & 4 & 30 \\
Bookcase   & 1 & 4 & 30 \\
Cube       & 1 & 4 & 60 \\
Cube       & 2 & 4 & 75 \\
2DBookcase & 1 & 4 & 180 \\
Dresser    & 1 & 4 & 100
    \end{tabular}
    \caption{Data for expert \fabplans.}
    \label{tab:expert-table}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/expertPlans-PLACEHOLDER.png}
    \caption{The optimal \fabplans for different projects, as generated by experts.}
    \label{fig:expert-results}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/expertVsPareto-PLACEHOLDER.png}
    \caption{Comparing each optimal \fabplan to our pareto front, computed over joint design and fabrication variations}
    \label{fig:expert-vs-pareto}
\end{figure}


We want to know if our tool can produce results that are at least as good as expert \fabplans, if not better.
\amy{"Experts are the current state-of-the-art for creating design variations and their optimal \fabplans."}

For each model, we asked experts to generate some design variations and \fabplans.
Figure \ref{fig:expert-results} shows the resulting designs, as well as the associated cost of each 
packing and cutting order.
\amy{We should compare our tool's results... if we can. Also, how to fit multiple variations?}

Because there are not enough points, 
we are unable to generate a Pareto front for the experts' plans 
--- an inherent advantage present in the programmatic approach.
Instead, we juxtapose the output of each method. 

Looking at the results in Figure \ref{fig:expert-vs-pareto},
our algorithm dominates the experts.
This is because, although expert plans seem sensible,
we are able to generate more design variations and \fabplans, 
including potentially unintuitive packing or cutting orders,
and evaluate them much more quickly than a human.
\amy{Optimizing cutting order is REALLY tedious for humans! Need to evaluate all possible reference points, and for angles, that might mean taking the time cost of setting up a different angle. But is that better than taking the precision loss across all n cuts? Also, expert \fabplans didn't vary that much/not very radical}
Additionally, our tool is considerably faster than the human experts, 
who on average spent 75 minutes creating their design variations.  
Overall, we are able to achieve equivalent optimization without the knowledge of a domain expert,
and much faster. Full detail of the expert plans is available in table \ref{tab:expert-table}. \adriana{How much of this time is spent actually designing? I'm not sure we can claim performance... but maybe... We may need to look a the results for this but what I'd like to say is: in all experiments we found solutions that have different trade-offs in x out of the y experiments we found solutions that dominate the experts designs (i.e. they are better in every metric). Again point to supplemental for all results and add the key ones here.}


\subsubsection{Performance Evaluation}
% Why do we care about brute force? What are we trying to show?
As a baseline, we first compare our implementation with a brute-force search approach.
The space of possible \fabplans grows exponentially, so brute force 
is tractable only for designs A and B, shown in Figure ~\ref{fig:comparison-brute-force}; we estimate the brute force runtime for all other designs.

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/comparison-brute-force.png}
    \caption{Comparison results between our methods and brute force method. The brute force methods mean that we randomly select a set of design variations. For each variation, we run Carpentry Compiler pipeline to generate its Pareto fronts \fabplans. Then we compare the two methods with running time and performance indicated with hypervolume metrics. There is only two simple, frame and long frames which are tractable with the brute force method.}
    \label{fig:comparison-brute-force}
\end{figure}


In order to assess the quality of our tool's \fabplans, we
use a metric called the \textit{hypervolume} ~\cite{auger2009theory}. % wondering whether we define this earlier or not
To calculate the hypervolume, we draw the smallest rectangular prism (axis-aligned, as per the L1 norm) 
between some reference point and each point on the pareto front.
We then union the volume of each shape to calculate the hypervolume.
Thus a larger hypervolume implies better \fabplans. \adriana{we talk about the hypervolume a lot, I moved this to the the background section. }
The pareto front that includes the origin therefore has the highest
possible hypervolume. 

% maybe there's a better mathematical way to express this?
% like closed neighborhood on the two points being compared

Figure \ref{fig:comparison-brute-force} indicates that for each design, our approach 
always beats out the brute force approach, and it reaches
the higher hypervolume much faster.

% Why?
Our tool has many obvious advantages over brute force.
Complete enumeration is very expensive,
and so the brute force method may not be able to 
discover the optimizations that our method ultimately
used in the final \fabplan. Also, in terms of resource usage,
... \amy{Are there other advantages?}

\paragraph{Performance estimate}
To estimate how long it might have taken a complete brute force solution, 
we measure the runtime of brute force methods on a subset $S$ of possible design variations $D$, then multiply that number by $\frac{\mid D \mid}{\mid S \mid}$ to find approximately how long it would take to optimize over all design variations. ... \todo{finish}

We also find that the hypervolume of the brute force approach is always equal to or less than that of our approach. Although we are using only a subset of design variations, the evidence suggests that ICEE approaches optimality. \amy{Maybe we could be stronger about this... or less strong, depending.}

\adriana{we also talked about the performance evaluation with taking the k designs that we end up exploring and comparing testings just those, the "Max" idea.}

\subsection{Performance Analysis and Ablation Study}
\amy{Sensitivity analysis?}
Finally, we assess the performance of \tool, end-to-end 
as well as of particular components.

%\paragraph{Computation Performance}
\paragraph{Performance Analysis}

%Computation time vs quality ( show this for at least 3 models of varying number of parts)  
%\begin{itemize}
%    \item figure of time vs hypervolume for all examples (just let it run until it tappers off.
%    \item table for each example number of parts, number design variations, number fab variations for a give design \# time when %the hypervolume  tapers off. discussion: size growns exponentially but our comp time does not.
%\end{itemize}


 \begin{figure*}
\centering
\includegraphics[width=\linewidth]{images/time-quality.png}
\caption{From left to right: 1) time versus \#e-nodes for populating e-graphs; 2) optimization time versus \#e-nodes; 3) relative hypervolume versus \#e-nodes.} 
\label{fig:time-quality}
\end{figure*}

% We want to know how long it takes for a certain "goodness"
We want to know how long it takes to produce a Pareto front 
whose hypervolume exceeds some threshold, i.e. when the 
line in figure \ref{fig:time-quality} tapers off.
Here, we choose the time that it takes to reach within
2\% of our final hypervolume.

Also of interest are various questions related to
expensive parts of our algorithm:
how long does it take to populate an e-graph, and how does
optimization time scale with the number of e-nodes?

These values are collected into table \ref{}.

Examining the table, we observe that our tool reaches 
very good results very quickly: on average,
it takes only about 60\% of the runtime to reach 98\% of the 
full runtime quality. This is on the scale of tens of seconds 
for all examples.

Another encouraging discovery is that as the size of the e-graph grows
exponentially, optimization time remains relatively stable, and even decreases.
This result suggests that our technique can scale to large or 
complex projects, and is bounded only be e-graph population.
\amy{What would be the right thing to conclude and how can we 
discuss ICEE here? Could we also conclude that we could optimize even more?}

\paragraph{Pruning Comparisons}
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/ablation-pruning-chair.jpg}
    \caption{Ablation test of pruning operator with the chair model.}
    \label{fig:ablation-pruning-chair}
\end{figure}
%Finally, we want to assess whether our proposed theoretical contributions were worthwhile. 
Finally, we want to examine the impact of various pruning schemes on the end-to-end result.
\amy{Why? Need to explain}

For the chair model, we ran \tool with three different pruning strategies \amy{How many experiments?},
and we note the end-to-end results generated, as a preliminary ablation study. 
\amy{Also, need to find an appropriate chart to present this many dimensions}
For each of (1) no pruning, (2) pruning via the creation of fresh e-graphs, and 
(3) pruning by removing e-classes, as described in Section \ref{sec:algorithm-overview},
we graphed the average hypervolume v.s. time (Figure \ref{fig:ablation-pruning-chair}).

The results indicate that strategy (1), no pruning, results in intractable growth
and time balloons without hypervolume increasing in proportion. 
We infer that pruning is essential, and without it, the growing number of 
 e-nodes and e-classes bloat the e-graph. We waste cycles
in searching and mutation, and the extra information is not valuable enough
to improve the hypervolume over pruning methods. In fact, it may prevent more
iterations of ICEE, which would otherwise move the pareto front closer to optimal.
We did not see a significant difference between strategies (2) and (3). 
\amy{What are the implications?}

%Table with average time and performance (hyper-volume)  for your algorithm and:
%\begin{itemize}
%    \item your method with no pruning ~\ref{fig:ablation-pruning-chair}
%    \item your method with no weight based selection (random)
%    \item rough to fine?
%\end{itemize}


\begin{itemize}
    \item nsg2 vs 3
    \item cut order
\end{itemize}


\subsection{Fabricated Results}
We have fabricate two models. For each model, we fabricate two design variations, shown in Figure ~\ref{fig:fabrication-result}. \haisen{used in teaser} 

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/fabrication-result.png}
    \caption{Fabrication results of two chair variations and two window variations.}
    \label{fig:fabrication-result}
\end{figure}

\subsection{Limitations and Future Work}

\adriana{Let's keep adding to this list as we go}

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{images/continuous-variation.png}
    \caption{Example of \fabplan optimization based on continuous variations generation of the input feasible design.}
    \label{fig:continuous-variation}
\end{figure}

Limitations and future work:
\chandra{1. key limitation is that we cannot guarantee that we will fully explore the space. in particular, if the space is too large and there is one design that achieves optimality, and we start from one that is far from it, we may not get to that good design. e.g. window 1.

2. our search space did not contain continuous variations. Good for FW. We could try to parallelize some parts of the implementation,

3. a. assembly: we also did not consider other cost metrics like assembly.
   b. minimized fab cost, but since we are exploring a joint design and fab space, we could consider
stability, strength, performance etc.

}

\begin{itemize}
    \item window 1 example
    \item Do not support free-form objects;
    \item No guarantees of convergence;
    \item Our current BOP E-graph could only encode discrete parameters. 
    Did not consider continuous variations; Figure ~\ref{fig:continuous-variation} shows one example that reduce the fabrication cost with tuning the continuous parameters of the input feasible design. 
    \item We apply the objective evaluation method in Carpentry Compiler which may not accuracy;
    \item Only consider subtractive approaches without additive process. We did not consider to merge multiple parts into one single part.
    \item Our framework could not guarantee to find better design variations than input design. For some models, we could not find any design variations whose fabrication cost is lower than that of the original design. For example XXX, the input model only use two kinds of parts. With our current evaluation method of fabrication cost, it tends to generate lower cost fabrication plans with less number of part types. 
    \item FW: Many steps in our algorithm can be parallel. In our current implementation, we did not do that.
    \item FW: We did not consider approximated part fabrication. During fabrication, if a part is almost what we want, we could just take it. Maybe we could save more material time and cost. Our current pipeline only consider small modification of design. During fabrication, we could also allow some fabricaiton error to improve cost further.   \item We did not consider approximated part fabrication. During fabrication, if a part is almost what we want, we could just take it. Maybe we could save more material time and cost. Our current pipeline only consider small modification of design. During fabrication, we could also allow some fabricaiton error to improve cost further.
   
\end{itemize}


Future work:
\begin{itemize}
    \item Future work: Assembly - take into account how assembly will happen when optimizing the design - make it easy to assemble and also structure stability. 
    \item Future work: Stability - different joint variations will affect the design stability. One interesting future work is to include stability measurement into our pipeline. We prefer to output structure-sound design variations with lower fabrication cost.
    \item Future work: include both continuous and joint variations to our framework.
    \item Extend the key idea of our pipeline to other domains. We only demonstrate our design and fabrication jointly encoding and optimization in carpentry domain. It's interesting to extend the idea to other fabrication process, such as additive which also involve a large design space and a multiple stage planning problems.
    
    \item We don't consider strength of the part in the
    pareto front. The chair is a good example
    of this---the one we pick may not be the strongest.
    \item consider branch and bound technique for multi-objective
    \item improve our current low-bound computation method
    
\end{itemize}
